Mixtape Application: Music Map Methodology and Evaluation

This report discusses dimensionality reduction techniques used to create a music map - a map where the distances between songs represent their similarity and that can be used to recommend songs. We evaluate two techniques: Isomap and L-Isomap.

==> Makefile <==
# 
# makefile para a compilação do documento
#
# Sáb Jun 23 21:13:37 BRT 2007
#

BASE_NAME = relatorio

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex 
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<
	$(PDFLATEX) $<
	evince $(BASE_NAME).pdf

$(BASE_NAME).ps: $(BASE_NAME).tex 
	$(LATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(LATEX) $< 
	$(LATEX) $<
	$(LATEX) $<
	
clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 


==> sections/dataset.tex <==
%\subsection{Datasets}\label{subsec:dataset}
\section{Last.fm Dataset}
\label{subsec:musicDatasets}

%\an{Rever se as figuras 1 e 2 incluem alguma informacao realmente relevante para o resto do artigo.}

In order to compute item-to-item similarity values, we rely on data from \url{Last.fm}, 
which is a social music site that tracks user musical tastes, finds
similar users, and provides music recommendations.


Our dataset was collected from November,
2014 to March, 2015, and contains 372,899 users (with their respective top-25
song lists), 2,060,173 songs, and 374,402 artists. Moreover, we also collected a
total of 1,006,236 user-generated tags, associated with songs. In particular, 75\% of songs have
had at least one associated tag in our dataset.




==> sections/related.tex <==
\chapter{Related Work}\label{sec:related}

\textbf{Large-scale information network embedding:} 
Dimensionality reduction is the transformation of high dimensional data into a
meaningful representation of reduced dimensionality, normally it is used to visualize
and analyze this data in a low-dimensional space and to avoid
undesirable effects of high dimensionality \cite{van2009dimensionality}.
The use of dimensionality reduction techniques can be applied to embed graphs and several classical methods of graph embedding and dimensionality reduction in general
can be found in literature, such as Multidimensional
Scaling (MDS) \cite{cox}, IsoMap \cite{TenenbaumEtAl2000} and Laplacian Eigenmap
\cite{Belkin:2003}, which time complexities are at least quadratic to the number
of vertices, which is too expensive for networks with millions
of nodes.  Some recent  studies describe techniques that aim to reduce computational complexity when considering very large information sets \cite{Ahmed:2013,Perozzi:2014,tang2015line}.
 

\textbf{Media item-to-item similarity computation:} 
Several research studies offer technical solutions to define similarity between a given pair of items, and they divide themselves among two schools. Some studies develop similarity measures that are based solely on content (objective approach), being that audio or video information—for instance, the spectral or rhythmic content of songs. On the other hand, other studies develop similarity measures that are based on user-generated data and tags, also known as collaborative filtering (subjective approach). In the context of music, 
different approaches to define item-to-item similarity have been studied extensively, such as content-based measures~\cite{mcfee2012learning, cano2005content, logan2001music,
flexer2014inter, aucouturier2005way, van2013deep},
that analyze spectral or rhythmic properties of
songs, and user-based
measures~\cite{minsu2015, konstas2009social, shepitsen2008personalized,
goussevskaia2008web, farrahi2014impact, kuhn2010social}, that
analyze user listening habits in online social networks or user-generated
tags~\cite{shepitsen2008personalized}.
Many of these studies aim at building recommendation
systems~\cite{mcfee2012learning, cano2005content,
van2013deep, farrahi2014impact, turnbull2014using, shepitsen2008personalized}.
In this work we adopt a cross-domain approach, combining information about user
listening habits and user-generated labels, such as tags and genres, to represent music similarity.

%%%%%%%%%%%%%%%%%%

\begin{comment}
\textbf{Content-similarity.} Many different research studies offer technical
solutions to define similarity between a given pair of items, and they divide
themselves among two schools. Some studies develop similarity measures that are
based solely on content, being that audio or video information - for instance,
the spectral or rhythmic content of songs - to define how similar they are.
\cite{logan2001music,mcfee2012learning,cano2005content}. On the other hand,
other studies develop similarity measures that are based on User data and human
tags \cite{konstas2009social,shepitsen2008personalized,kuhn2010social}.
%Our project explores a similarity measure based on the co-occurrence of pairs
% of items - songs, series or TV shows, amongst extensive usage data.


\begin{comment}
\textit{Embedding techniques: Isomap (global) nonlinear dimensionality
reduction~\cite{tenenbaum_global_2000}, LLE (local)~\cite{silva2002global}, LME (non-metric?), TSNE (long tail?)}

\end{comment}



